Online Knowledge Production in Polarized Political Memes: The Case of Critical Race Theory

Visual culture has long been deployed by actors across the political spectrum as tools of political mobilization, and have recently incorporated new communication tools, such as memes, GIFs, and emojis. In this study, we analyze the top-circulated Facebook memes relating to critical race theory (CRT) from May 2021 - May 2022 to investigate their visual and textual appeals. Using image clustering techniques and critical discourse analysis, we find that both pro- and anti-CRT memes deploy similar rhetorical tactics to make bifurcating arguments, most of which do not pertain to the academic formulations of CRT. Instead, these memes manipulate definitions of racism and antiracism to appeal to their respective audiences. We argue that labeling such discursive practices as simply a symptom of "post-truth" politics is a potentially unproductive stance. Instead, theorizing the knowledge-building practices of these memes through a lens of political epistemology allows us to understand how they produce meaning.

==> xx-unused-text.tex <==
%in the case of word filters, users define their preferences via  which, when occurring, results in content being blocked. On the other hand, the text descriptions that platforms offer to explain
%End-users rely on words to make sense of, communicate, and adjust their preferences in current text-based personal moderation tools. In rule-based interfaces such as word filters, users define a list of blocked keywords. 

%In  approaches such as toxicity toggle or sliders, users configure the moderation settings based on their understanding of the meanings of terminology used in the interfaces. However, words can be ambiguous and limited. 
% to mediate the communication between users and the personal moderation systems. 
%The limitation of the communication mechanism between users and the personal moderation systems, in turn, result in gaps between users' mental model and system's model, which further prevent users from customizing moderation settings at their desired levels of granularity. 




% These examples demonstrated the subjectivity of toxicity and the challenge of moderating content using a simple one-size-fit-all tool. At the extreme end, participants expressed desires to make decisions on a case by case level. Overall, our participants speak to the need of more granular level of control, which can allow customization on a more personal level. 


% not sure how to make transition between the two sections
% \subsubsection{Desire transparency in meanings of toxicity}


% Transparency is also desired because it allows users to be aware of the potential bias in moderation systems, which is especially valued by participants given how varied the preferences for moderation settings differ across individuals. In our interviews, many participants reported concerns of implicit bias in moderation systems. For example, P3 said: 
% \begin{quote}
% ``\textit{If like everyone has their own conception of how things should be ranked, I guess I'd be curious, like who this was based on, like how are these calculated? }'' - P3 
% \end{quote}


% Points:
% - Participants desire control in all the moderation modes: toggle, category sliders, topic sliders
%     - Changes in number of levels (+ or -)
%          - Toggle buttons too extreme
%     - Additional topics in intel slider
% - Transparency is an important prerequisite of control
%     - Need understanding of "toxic" in category sliders
%     - Need more details about intel filters
% - Labor is a counter to control 
%     - Word filters are hard to make and tune
%     - too many levels on scales make it hard to interpret differences
%

% Transparency was also an important factor for participants when determining when the degree of control was inadequate. For example, one participant called to attention a limitation in control as a result of the Intel slider providing transparency into the specific categories of toxicity:
% \begin{quote}
%     \textit{``I'm also wondering if it's not a good idea to have categories, because of the exclusion, because then just by going into the settings yourself and saying `Oh, well, my thing isn't there.' You're, like, being discriminated against.''} - P22
% \end{quote}

% Finally, participants noted that while control over moderation was generally desirable, there was a trade-off between the amount of labor they were willing to spend versus how effective they perceived the controls to be over their experiences. P2 noted that:
% \begin{quote}
%     \textit{``[...] the more effort I invest into something, like the more time I spend, for example, in curating my Twitter feed, the more irritated I get when I get things on my feed that I didn't want.''} - P22
% \end{quote} 

% More control often also requires a higher amount of effort invested in interpreting the various settings that can be controlled. (...?)
% Q: Maybe move this to sec. below?







%the platform must clearly define these categories and communicate these definitions to the users so that the latter can align their mental model with that of the system. However, existing personal moderation tools largely resort to text descriptions for explaining what the controls for moderation are and how they work. For example, a category-based control might be designated simply as \textit{``hate speech''} or levels on a scale denoted as \textit{``more toxic''} or \textit{``less toxic''}. While these descriptions are simple and perhaps the best that platform designers have come up with yet to describe the behavior of their classifier, they limit users' ability to build an accurate and sufficiently detailed mental model of the moderation system. We found in our interviews that such abstract terminology is often ambiguous to participants, who expressed a desire for greater clarity around the meanings of various terms and the distinctions between different categories and levels. 



%Even categories that are seemingly more specific, such as the n-word toggle used in Intel's category-based controls, can be ambiguous in different contexts. 
%While its operationalization is crisp---either a comment has or does not have the n-word---some participants speculated that the use of n-word may not be offensive when used within African-American communities and should therefore be allowed, whereas others argued for removing any comment containing the n-word. 
%Since not everyone agrees on how the system should handle the use of n-word, this category still raises challenges to building a common mental model. A personal moderation setting that makes sense to one group of users can be hard to navigate for another group. 



\subsubsection{User Mental Models for Performance Trade-offs: Intensity and Proportion Filters}

% When engaging with intensity and probability filters, most participants noticed that even at stricter moderation settings, probability filters did not remove a few particularly toxic comments, whereas intensity filters removed those comments. This demonstrates that there is at least some correlation between our moderation system's operationalization of toxicity and participants' perceptions of inappropriateness in comments.

Moderation systems based on machine learning systems often require users to consider trade-offs. However, to effectively decide the thresholds for these trade-offs, users need to form a mental model of what trade-offs are being made.  We examine aspects of this through comparing the participants' experiences configuration of moderation via differently grounded scales: intensity-based scales--those where the tool removed comments as toxic as or more toxic than the configured level (from \textit{`Nothing'} to \textit{`Very Toxic'}), and proportion-based scales--those where the tool impacted a larger proportion of comments based on the configured level (from \textit{`No Moderation'} to \textit{`A Lot of Moderation'}). 

Participants invariably inquired how the two filters differed in the properties that affected the algorithms' decision making. After our explanation and comparing the two filters' outputs, most participants showed preference for using intensity-based scales to configure filters compared to proportion-based ones. Participants were observed to be less tolerant towards false-negatives, with () noting that they noticed a few particularly toxic comments were being missed even when allowing a higher proportional impact on their feed, while setting the intensity threshold removed those comments.

Even though they recognized that their perceptions of inappropriateness may not perfectly align with the moderation system's, they felt that the graduated removals of intensity filters would regulate the most blatantly inappropriate posts at their chosen setting. Along the same lines, participants  characterized the indeterminate removals of proportion filter `confusing' or having `lack of clarity.' P13 worried that this filter would incorrectly remove comments that he would rather like to see. 
P2 felt that even if the proportion filter removes nine out of ten toxic comments, one remaining comment that is personally hurtful to her may negate its utility.
Similarly, participant P3 said:

\begin{quote}
    \textit{``I think there are particular things that I feel really strongly about. Like, I do not want to see any racial slurs on my feed or ethnic slurs. And so I guess I just would rather not see it versus if this is just reducing the amount of bad stuff, it might be that the things that are slipping through are those that I find really offensive. And the things that are randomly getting chosen to be removed are like mildly offensive. And I guess, I really want a certain subset of really offensive stuff just off my feed.''} - P3
\end{quote}

% \begin{quote}
%     \textit{``Even if you remove nine out of 10 toxic comments, but the last one is incredibly harmful to me personally or it's just extremely toxic, it kind of negates taking out the other nine. So I don't think quantity is the way to go with this. I think quality is.''} - P2
% \end{quote}

On the other hand, Participants P17 and P21 considered the concept of \textit{toxicity} to be quite abstract or subjective, and therefore preferred the probability filters over intensity filters. P17 preferred that the former lets in comments that may be considered toxic by some, but users may adjust the frequency of such comments depending on how vulnerable they feel in the moment. He also expressed lack of confidence in the intensity filter's ability to accurately grade toxicity levels. Similarly, Participant P21 said:

\begin{quote}
    \textit{``I think a lot of people might not want to see particular words, phrases or messages, and intensity filter would be perfect for them, but for somebody like myself who just maybe wanted to decrease the amount of negativity by just a little bit, I think probability filters would be more fitting because it's making less of a judgment call about the posts, it's just grabbing some that it deems to be negative.''} - P21
\end{quote}


\subsection{Exerting Control Over Moderation Systems}

Many participants desired more control over the details of their moderation configurations. However, the gap between users' mental model and systems' operations limited their ability to exert control. This gap manifested in two ways: (1) criteria for control: personal moderation systems often did not distinguish content along criteria that users desired or cared about; (2) granularity of control: personal moderation systems sometimes offered insufficient granularity or granularity on controls without corresponding clarity on their effectiveness. 

\subsubsection{Criteria for Control}

When we showed different moderation interfaces to participants, a general theme we noticed is that participants found the descriptions and terms used to define moderation settings (categories and levels) to often be ambiguous or subjective. 

Additionally, participants could desire ways to control the system that are not afforded by the system. P3, while working through the category based filters, said she would want a combination of toxic content to be filtered out, not just one or the other based on toxicity defined by the system. 
\begin{quote}
    \textit{``Yeah I mean and maybe that's kind of an impossible problem to solve...it's like everyone has their own conception of how things are.''- P3}
\end{quote}

These mismatches between the type of control desired and the control actually afforded can even become a source of exclusion for some:
\begin{quote}
  \textit{``I'm also wondering if it's not a good idea to have categories, because of the exclusion, because then just by going into the settings yourself and saying `Oh, well, my thing isn't there.' You're, like, being discriminated against.''} - P22
\end{quote}
